A Survey on Open Information Extraction from Rule-based Model to Large Language Model

Open Information Extraction (OpenIE) represents a crucial NLP task aimed at deriving structured information from unstructured text, unrestricted by relation type or domain. This survey paper provides an overview of OpenIE technologies spanning from 2007 to 2024, emphasizing a chronological perspective absent in prior surveys. It examines the evolution of task settings in OpenIE to align with the advances in recent technologies. The paper categorizes OpenIE approaches into rule-based, neural, and pre-trained large language models, discussing each within a chronological framework. Additionally, it highlights prevalent datasets and evaluation metrics currently in use. Building on this extensive review, the paper outlines potential future directions in terms of datasets, information sources, output formats, methodologies, and evaluation metrics.

==> content/acknowledgements.tex <==
% \section*{Acknowledgements}

% The work was supported  in part by Alibaba Innovative Research (AIR) project support funding. We thank Yafu Li and all reviewers for their generous help and advice during this research. 
% This work was supported in part by the US Department of Defense under the DARPA CCU program. Any opinions expressed herein are those of the authors and do not necessarily reflect the views of the U.S. Department of Defense or the U.S. Government.

